Using super-resolution for enhancing visual perception and segmentation performance in veterinary cytology

The primary objective of this research was to enhance the quality of semantic segmentation in cytology images by incorporating super-resolution (SR) architectures. An additional contribution was the development of a novel dataset aimed at improving imaging quality in the presence of inaccurate focus. Our experimental results demonstrate that the integration of SR techniques into the segmentation pipeline can lead to a significant improvement of up to 25% in the mean average precision (mAP) segmentation metric. These findings suggest that leveraging SR architectures holds great promise for advancing the state of the art in cytology image analysis.

==> bibliography.tex <==
@INPROCEEDINGS{dual_sr_segm,
  author={Wang, Li and Li, Dong and Zhu, Yousong and Tian, Lu and Shan, Yi},
  booktitle={2020 IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)}, 
  title={Dual Super-Resolution Learning for Semantic Segmentation}, 
  year={2020},
  volume={},
  number={},
  pages={3773-3782}}
  
  @inproceedings{how_effective,
author = {Pereira, Matheus and dos Santos, Jefersson},
year = {2019},
month = {10},
pages = {202-209},
title = {How Effective Is Super-Resolution to Improve Dense Labelling of Coarse Resolution Imagery?}
}

@INPROCEEDINGS{mri,  author={Pham, C.-H. and Tor-Díez, C. and Meunier, H. and Bednarek, N. and Fablet, R. and Passat, N. and Rousseau, F.},  booktitle={2019 IEEE 16th International Symposium on Biomedical Imaging (ISBI 2019)},   title={Simultaneous Super-Resolution and Segmentation Using a Generative Adversarial Network: Application to Neonatal Brain MRI},   year={2019},  volume={},  number={},  pages={991-994}}



@Article{app11167181,
AUTHOR = {Caputa, Jakub and \L{}ukasik, Daria and Wielgosz, Maciej and Karwatowski, Micha\l{} and Fr\k{a}czek, Rafa\l{} and Russek, Pawe\l{} and Wiatr, Kazimierz
},
TITLE = {Fast Pre-Diagnosis of Neoplastic Changes in Cytology Images Using Machine Learning},
JOURNAL = {Applied Sciences},
VOLUME = {11},
YEAR = {2021},
NUMBER = {16},
ARTICLE-NUMBER = {7181},
URL = {https://www.mdpi.com/2076-3417/11/16/7181},
ISSN = {2076-3417},
ABSTRACT = {We present the experiment results to use the YOLOv3 neural network architecture to automatically detect tumor cells in cytological samples taken from the skin in canines. A rich dataset of 1219 smeared sample images with 28,149 objects was gathered and annotated by the vet doctor to perform the experiments. It covers three types of common round cell neoplasms: mastocytoma, histiocytoma, and lymphoma. The dataset has been thoroughly described in the paper and is publicly available. The YOLOv3 neural network architecture was trained using various schemes involving original dataset modification and the different model parameters. The experiments showed that the prototype model achieved 0.7416 mAP, which outperforms the state-of-the-art machine learning and human estimated results. We also provided a series of analyses that may facilitate ML-based solutions by casting more light on some aspects of its performance. We also presented the main discrepancies between ML-based and human-based diagnoses. This outline may help depict the scenarios and how the automated tools may support the diagnosis process.},
DOI = {10.3390/app11167181}
}


@INPROCEEDINGS{9908709,
  author={Mazurek, Szymon and Wielgosz, Maciej and Caputa, Jakub and Fr\k{a}czek, Rafa\l{} and Karwatowski, Micha\l{} and Grzeszczyk, Jakub and \L{}ukasik, Daria and \'S{}miech, Anna and Russek, Pawe\l{} and Jamro, Ernest and D\k{a}browska-Boruch, Agnieszka and Pietro\'n, Marcin and Koryciak, Sebastian and Wiatr, Kazimierz
},
  booktitle={2022 17th Conference on Computer Science and Intelligence Systems (FedCSIS)}, 
  title={Canine age classification using Deep Learning as a step toward preventive medicine in animals}, 
  year={2022},
  volume={},
  number={},
  pages={169-172},
  doi={10.15439/2022F226}}


@misc{sr_dataset,
    title = {{Super Resolution data set}},
    howpublished = {\url{https://git.plgrid.pl/projects/CYFROVET/repos/dataset-super-resolution/browse}},
}


@misc{swin_transformer,

  
  author = {Liu, Ze and Lin, Yutong and Cao, Yue and Hu, Han and Wei, Yixuan and Zhang, Zheng and Lin, Stephen and Guo, Baining},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Swin Transformer: Hierarchical Vision Transformer using Shifted Windows},
  
  publisher = {arXiv},
  
  year = {2021},
  
  copyright = {Creative Commons Attribution 4.0 International}
}



@misc{casmrcnn,
  

  
  author = {Cai, Zhaowei and Vasconcelos, Nuno},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Cascade R-CNN: High Quality Object Detection and Instance Segmentation},
  
  publisher = {arXiv},
  
  year = {2019},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{resnest,

  
  author = {Zhang, Hang and Wu, Chongruo and Zhang, Zhongyue and Zhu, Yi and Lin, Haibin and Zhang, Zhi and Sun, Yue and He, Tong and Mueller, Jonas and Manmatha, R. and Li, Mu and Smola, Alexander},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {ResNeSt: Split-Attention Networks},
  
  publisher = {arXiv},
  
  year = {2020},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{coco,
  author = {Lin, Tsung-Yi and Maire, Michael and Belongie, Serge and Bourdev, Lubomir and Girshick, Ross and Hays, James and Perona, Pietro and Ramanan, Deva and Zitnick, C. Lawrence and Dollár, Piotr},
  
  keywords = {Computer Vision and Pattern Recognition (cs.CV), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Microsoft COCO: Common Objects in Context},
  
  publisher = {arXiv},
  
  year = {2014},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@misc{cyfronet,
    title = {{Prometheus Supercomputer}},
    howpublished = {\url{https://kdm.cyfronet.pl/portal/Prometheus:Podstawy}},
}

@misc{grzeszczyk2023segmentation,
      title={Segmentation of the veterinary cytological images for fast neoplastic tumors diagnosis}, 
      author={Jakub Grzeszczyk and Micha\l{} Karwatowski and \L{}ukasik, Daria and Maciej Wielgosz and Pawe\l{} Russek and Szymon Mazurek and Jakub Caputa and Rafa\l{} Fr\k{a}czek and \'S{}miech, Anna and Ernest Jamro and Sebastian Koryciak and Agnieszka D\k{a}browska-Boruch and Pietro\'n, Marcin and Kazimierz Wiatr
},
      year={2023},
      eprint={2305.04332},
      archivePrefix={arXiv},
      primaryClass={cs.CV}
}
